Bring Your Own Codegen to Deep Learning Compiler

Deep neural networks (DNNs) have been ubiquitously applied in many applications, and accelerators are emerged as an enabler to support the fast and efficient inference tasks of these applications. However, to achieve high model coverage with high performance, each accelerator vendor has to develop a full compiler stack to ingest, optimize, and execute the DNNs. This poses significant challenges in the development and maintenance of the software stack. In addition, the vendors have to contiguously update their hardware and/or software to cope with the rapid evolution of the DNN model architectures and operators. To address these issues, this paper proposes an open source framework that enables users to only concentrate on the development of their proprietary code generation tools by reusing as many as possible components in the existing deep learning compilers. Our framework provides users flexible and easy-to-use interfaces to partition their models into segments that can be executed on "the best" processors to take advantage of the powerful computation capability of accelerators. Our case study shows that our framework has been deployed in multiple commercial vendors' compiler stacks with only a few thousand lines of code.

==> figures/fig-quantize.tex <==
\begin{figure}[tbh]
	\centering
    \includegraphics[width=0.75\textwidth]{./figures/source/quantize.pdf}
    \caption{An example of a deep learning model with partial quantization. \textit{\texttt{Q}} is a sequence of operators for (de)quantization inserted by the accelerator backend.}
	\label{fig:quantize}
\end{figure}

==> figures/fig-trt-init-ssd.tex <==
\begin{figure}[tbh]
	\centering
    \includegraphics[width=\linewidth]{./figures/source/trt-init-ssd.pdf}
    \caption{The TensorRT engine initialization time of each kernel in SSD 512 MobileNet 1.0 on NVIDIA Jetson Xavier. The x-axis also shows the speedup of each subgraph over the TVM baseline.}
	\label{fig:trt-init-ssd}
\end{figure}

==> table/tensorrt-fp16.tex <==
\begin{table}[tbh]
\centering
\caption{End-to-end performance of half-precision models on NVIDIA Jetson Xavier with TensorRT.}
\label{tbl:trt-fp16}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Model} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Latency\\ (ms)\end{tabular}} &
  \multirow{2}{*}{Speedup} &
  \multicolumn{2}{c}{Offload Ratio (\%)} \\ \cline{4-5}
                          &          &      & Node & MAC \\ \hline
ResNet-18                 & 2.14     & 2.06$\times$ & 100\% & 100\% \\ \hline
ResNet-50 v1b/v2          & 4.12     & 3.58$\times$ & 100\% & 100\% \\ \hline
Inception V3              & 6.10     & 5.30$\times$ & 100\% & 100\% \\ \hline
DarkNet-53                & 5.43     & 8.81$\times$ & 100\% & 100\% \\ \hline
MobileNet V2 1.0          & 2.22     & 1.78$\times$ & 100\% & 100\% \\ \hline
VGG19                     & 9.78     & 2.29$\times$ & 100\% & 100\% \\ \hline
SSD 512 MobileNet 1.0     & 11.06 & 3.73$\times$ & 36\% & 100\%     \\ \hline
SSD 300 ResNet-34         & 15.29 & 108.68$\times$ & 41\% & 100\%     \\ \hline
Faster R-CNN ResNet50 v1b & 99.72 & 25.53$\times$ & 63\% & 100\%     \\ \hline
\end{tabular}%
}
\end{table}

==> table/tensorrt-fp32.tex <==
\begin{table}[tbh]
\centering
\caption{End-to-end performance of full precision models on NVIDIA Jetson Xavier with TensorRT.}
\label{tbl:trt-fp32}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Model} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Latency\\ (ms)\end{tabular}} &
  \multirow{2}{*}{Speedup} &
  \multicolumn{2}{c}{Offload Ratio (\%)} \\ \cline{4-5}
                          &          &      & Node & MAC \\ \hline
ResNet-18                 & 4.12     & 1.07$\times$ & 100\% & 100\% \\ \hline
ResNet-50 v1b/v2          & 9.66     & 1.53$\times$ & 100\% & 100\% \\ \hline
Inception V3              & 16.13    & 2.00$\times$ & 100\% & 100\% \\ \hline
DarkNet-53                & 12.81    & 3.73$\times$ & 100\% & 100\% \\ \hline
MobileNet V2 1.0          & 3.32     & 1.19$\times$ & 100\% & 100\% \\ \hline
VGG19                     & 24.26    & 0.92$\times$ & 100\% & 100\% \\ \hline
SSD 512 MobileNet 1.0     & 18.43    & 2.24$\times$ & 36\% & 100\%     \\ \hline
SSD 300 ResNet-34         & 34.31    & 48.44$\times$ & 41\% & 100\%     \\ \hline
Faster R-CNN ResNet50 v1b & 404.51   & 6.29$\times$ & 63\% & 100\%     \\ \hline
\end{tabular}%
}
\end{table}
